Bridging the Covid-19 Data and the Epidemiological Model using Time-Varying Parameter SIRD Model

This paper extends the canonical model of epidemiology, the SIRD model, to allow for time-varying parameters for real-time measurement and prediction of the trajectory of the Covid-19 pandemic. Time variation in model parameters is captured using the generalized autoregressive score modeling structure designed for the typical daily count data related to the pandemic. The resulting specification permits a flexible yet parsimonious model with a low computational cost. The model is extended to allow for unreported cases using a mixed-frequency setting. Results suggest that these cases' effects on the parameter estimates might be sizeable. Full sample results show that the flexible framework accurately captures the successive waves of the pandemic. A real-time exercise indicates that the proposed structure delivers timely and precise information on the pandemic's current stance. This superior performance, in turn, transforms into accurate predictions of the confirmed and death cases.

==> Tables/Table_ForecastHubModels.tex <==
    \begin{tabular}{|l|l|r|}
          Abbreviation & Team & Forecast  \\   \hline  \hline
        AIpert-pwllnod  & AIpert.org team  & 68  \\
        BPagano-RtDriven  & BPagano  & 91  \\ 
        CovidAnalytics-DELPHI  & CovidAnalytics at MIT  & 111  \\ 
        COVIDhub-4\_week\_ensemble  & COVID-19 Forecast Hub  & 111  \\ 
        COVIDhub-baseline  & COVID-19 Forecast Hub  & 156  \\ 
        COVIDhub-ensemble  & COVID-19 Forecast Hub  & 114  \\ 
        COVIDhub-trained\_ensemble  & COVID-19 Forecast Hub  & 62  \\ 
        CU-select  & Columbia University  & 142  \\ 
        DDS-NBDS  & Discrete Dynamical Systems  & 94  \\ 
        epiforecasts-ensemble1  & EpiForecasts group at the London School of Hygiene   &  \\ 
                                & Tropical Medicine  & 92  \\ 
        GT-DeepCOVID  & GT  & 111  \\ 
        IEM\_MED-CovidProject  & IEM MED  & 71  \\ 
        JHU\_CSSE-DECOM  & Johns Hopkins Center for Systems Science and Engineering  & 74  \\ 
        JHU\_IDD-CovidSP & Johns Hopkins ID Dynamics COVID-19 Working Group  & 99  \\ 
        JHUAPL-Bucky  & Johns Hopkins University Applied Physics Lab  & 92  \\ 
        Karlen-pypm  & Karlen Working Group  & 94  \\ 
        KITmetricslab-select\_ensemble  & KITmetricslab  & 57  \\ 
        Microsoft-DeepSTIA  & Microsoft  & 72  \\ 
        MIT\_CritData-GBCF  & MIT-CriticalData  & 88  \\ 
        MIT\_ISOLAT-Mixtures  & IDSS COVID-19 Collaboration (Isolat) at MIT  & 71  \\  
        MIT-Cassandra  & MIT-Cassandra  & 59  \\  
        MOBS-GLEAM\_COVID  & MOBS Lab at Northeastern  & 117  \\  
        MUNI-ARIMA  & Masaryk University  & 55  \\  
        PSI-DRAFT  & Predictive Science Inc  & 109  \\  
        RobertWalraven-ESG  & Robert Walraven  & 112  \\  
        SteveMcConnell-CovidComplete  & Steve McConnell  & 100  \\ 
        UCSD\_NEU-DeepGLEAM  & UCSD\_NEU  & 87  \\  
        UMass-MechBayes  & UMass-Amherst  & 102  \\  
        UMich-RidgeTfReg  & The University of Michigan  & 89  \\  
        USC-SI\_kJalpha & University of Southern California  & 131  \\  \hline \hline
 \end{tabular}
